Deep Reinforcement Learning for Autonomous Cyber Defence: A Survey

The rapid increase in the number of cyber-attacks in recent years raises the need for principled methods for defending networks against malicious actors. Deep reinforcement learning (DRL) has emerged as a promising approach for mitigating these attacks. However, while DRL has shown much potential for cyber defence, numerous challenges must be overcome before DRL can be applied to the autonomous cyber defence (ACD) problem at scale. Principled methods are required for environments that confront learners with very high-dimensional state spaces, large multi-discrete action spaces, and adversarial learning. Recent works have reported success in solving these problems individually. There have also been impressive engineering efforts towards solving all three for real-time strategy games. However, applying DRL to the full ACD problem remains an open challenge. Here, we survey the relevant DRL literature and conceptualize an idealised ACD-DRL agent. We provide: i.) A summary of the domain properties that define the ACD problem; ii.) A comprehensive comparison of current ACD environments used for benchmarking DRL approaches; iii.) An overview of state-of-the-art approaches for scaling DRL to domains that confront learners with the curse of dimensionality, and; iv.) A survey and critique of current methods for limiting the exploitability of agents within adversarial settings from the perspective of ACD. We conclude with open research questions that we hope will motivate future directions for researchers and practitioners working on ACD.

==> inc/makebigenvtable.tex <==
\usepackage{csvsimple,filecontents}
\usepackage{graphicx}
\usepackage{multirow}
\usepackage{amsfonts}
\usepackage{xstring}
\usepackage{amsmath}
\usepackage{pgffor}

\newcommand{\xmark}{\text{\sffamily X}}
\newcommand{\convert}[1]{%
    \IfEqCase{#1}{%
        {Y}{\checkmark}%
        {N}{\xmark}%
        {C}{$\nearrow$}%
        % you can add more cases here as desired
    }[{\rotatebox[origin=c]{90}{\ \textbf{#1}\ }}]% Assumption, if it is not one of the above cases, then it is a header...
}%
\newcommand{\pconvert}[1]{%
    \IfEqCase{#1}{%
        {Name}{\textbf{Name}}%
        % you can add more cases here as desired
    }[#1] % Return unmodified 
}%

%-------------------------------------------------------------------------------------------

\providecommand{\insertRows}[3]{
\multirow{#2}{3cm}{\textbf{#1}} 
\csvreader[head to column names, 
           late after line=\\\cline{2-\clineend},
           filter expr={
           test{\ifnumless{\thecsvinputline}{#3}}
         }]%
{\filepath}{}%
{\columns}%
}

%-------------------------------------------------------------------------------------------

\providecommand{\insertOffsetRows}[4]{
\multirow{#2}{3cm}{\textbf{#1}}
\csvreader[head to column names,
           late after line=\\\cline{2-{\clineend}},
           filter expr={
               test{\ifnumgreater{\thecsvinputline}{#3}}
               and test{\ifnumless{\thecsvinputline}{#4}}
         }]%
{\filepath}{}%
{\columns }%
}

%-------------------------------------------------------------------------------------------

\newcommand{\maketable}{
%\begin{tabular}{|l|l||l|l|l|l|}%
\begin{tabular}{|l|l|\columnsspec}%
\hline
\multicolumn{\clineend}{|c|}{\textbf{\tabletitle}} \\
\hline
\multicolumn{2}{|c||}{\textbf{Categories}} & 
\multicolumn{3}{|c||}{\textbf{ACO}} &
\multicolumn{5}{|c||}{\textbf{NBD}} &
\multicolumn{8}{|c||}{\textbf{GD2D}} &
\multicolumn{3}{|c||}{\textbf{DCC}} &
\multicolumn{3}{|c||}{\textbf{RS}} &
\multicolumn{3}{|c|}{\textbf{MG}} \\
\hline
\insertRows{General}{2}{4}
\hline
\hline
%------------------------------------------------------
\insertOffsetRows{Environment Properties}{5}{3}{9}
\hline
\hline
%------------------------------------------------------
\insertOffsetRows{Observation Properties}{4}{8}{13}
\hline
\hline
%------------------------------------------------------
\insertOffsetRows{Action Properties}{4}{12}{17}
\hline
\hline
\end{tabular}}

%-------------------------------------------------------------------------------------------


==> inc/makeenvtable.tex <==
\usepackage{csvsimple,filecontents}
\usepackage{multirow}
\usepackage{amsfonts}
\usepackage{xstring}
\usepackage{amsmath}
\usepackage{pgffor}

\newcommand{\xmark}{\text{\sffamily X}}
\newcommand{\convert}[1]{%
    \IfEqCase{#1}{%
        {Y}{\checkmark}%
        {N}{\xmark}%
        {C}{$\nearrow$}%
        % you can add more cases here as desired
    }[\textbf{#1}]% Assumption, if it is not one of the above cases, then it is a header...
}%
\newcommand{\pconvert}[1]{%
    \IfEqCase{#1}{%
        {Environment Name}{\textbf{Environment Name}}%
        % you can add more cases here as desired
    }[#1] % Return unmodified 
}%

%-------------------------------------------------------------------------------------------

\providecommand{\insertRows}[1]{
%\multirow{#2}{3cm}{\textbf{#1}} 
\csvreader[head to column names, 
late after line=\\\hline, %\cline{1-\clineend},
filter expr={test{\ifnumless{\thecsvinputline}{#1}}}]%
{\filepath}{}%
{\columns}%
}

%-------------------------------------------------------------------------------------------

%\providecommand{\insertOffsetRows}[4]{
%\multirow{#2}{3cm}{\textbf{#1}}
%\csvreader[head to column names,
%           late after line=\\\cline{2-{\clineend}},
%           filter expr={
%               test{\ifnumgreater{\thecsvinputline}{#3}}
%               and test{\ifnumless{\thecsvinputline}{#4}}
%         }]%
%{\filepath}{}%
%{\columns }%
%}

%-------------------------------------------------------------------------------------------

\newcommand{\maketable}{
%\begin{tabular}{|l|l||l|l|l|l|}%
\begin{tabular}{|l|\columnsspec}%
\hline
\multicolumn{\clineend}{|c|}{\textbf{\tabletitle}}\\
\hline
\hline
\insertRows{14}
%\hline
\hline
%------------------------------------------------------
%\insertOffsetRows{Environment Properties}{5}{3}{9}
%\hline
%\hline
%------------------------------------------------------
%\insertOffsetRows{Observation Properties}{4}{8}{13}
%\hline
%\hline
%------------------------------------------------------
%\insertOffsetRows{Action Properties}{4}{12}{17}
%\hline
%\hline
\end{tabular}}

%-------------------------------------------------------------------------------------------


==> inc/makeenvtable10.tex <==
\usepackage{csvsimple,filecontents}
\usepackage{multirow}
\usepackage{xstring}
\usepackage{amsfonts}
\usepackage{amsmath}

\newcommand{\xmark}{\text{\sffamily X}}
\newcommand{\convert}[1]{%
    \IfEqCase{#1}{%
        {Y}{\checkmark}%
        {N}{\xmark}%
        {C}{$\nearrow$}%
        % you can add more cases here as desired
    }[\textbf{#1}]% Assumption, if it is not one of the above cases, then it is a header...
}%
\newcommand{\pconvert}[1]{%
    \IfEqCase{#1}{%
        {Name}{\textbf{Name}}%
        % you can add more cases here as desired
    }[#1] % Return unmodified 
}%

%-------------------------------------------------------------------------------------------

\providecommand{\insertRows}[3]{
\multirow{#2}{3cm}{\textbf{#1}} 
\csvreader[head to column names, 
           late after line=\\\cline{2-10},
           filter expr={
           test{\ifnumless{\thecsvinputline}{#3}}
         }]%
{\filepath}{}%
{\columns}%
}

%-------------------------------------------------------------------------------------------

\providecommand{\insertOffsetRows}[4]{
\multirow{#2}{3cm}{\textbf{#1}}
\csvreader[head to column names,
           late after line=\\\cline{2-10},
           filter expr={
               test{\ifnumgreater{\thecsvinputline}{#3}}
               and test{\ifnumless{\thecsvinputline}{#4}}
         }]%
{\filepath}{}%
{\columns }%
}

%-------------------------------------------------------------------------------------------

\newcommand{\maketable}{
\begin{tabular}{|l|l||l|l|l|l|l|l|l|l|}%
\hline
\multicolumn{10}{|c|}{\textbf{\tabletitle}} \\
\hline
\insertRows{General}{2}{4}
\hline
\hline
%------------------------------------------------------
\insertOffsetRows{Environment Properties}{5}{3}{9}
\hline
\hline
%------------------------------------------------------
\insertOffsetRows{Observation Properties}{4}{8}{13}
\hline
\hline
%------------------------------------------------------
\insertOffsetRows{Action Properties}{4}{12}{17}
\hline
\hline
\end{tabular}}

%-------------------------------------------------------------------------------------------


==> inc/makeenvtable5.tex <==
\usepackage{csvsimple,filecontents}
\usepackage{multirow}
\usepackage{xstring}
\usepackage{amsfonts}
\usepackage{amsmath}

\newcommand{\xmark}{\text{\sffamily X}}
\newcommand{\convert}[1]{%
    \IfEqCase{#1}{%
        {Y}{\checkmark}%
        {N}{\xmark}%
        {C}{$\nearrow$}%
        % you can add more cases here as desired
    }[\textbf{#1}]% Assumption, if it is not one of the above cases, then it is a header...
}%
\newcommand{\pconvert}[1]{%
    \IfEqCase{#1}{%
        {Name}{\textbf{Name}}%
        % you can add more cases here as desired
    }[#1] % Return unmodified 
}%

%-------------------------------------------------------------------------------------------

\providecommand{\insertRows}[3]{
\multirow{#2}{3cm}{\textbf{#1}} 
\csvreader[head to column names, 
           late after line=\\\cline{2-5},
           filter expr={
           test{\ifnumless{\thecsvinputline}{#3}}
         }]%
{\filepath}{}%
{\columns}%
}

%-------------------------------------------------------------------------------------------

\providecommand{\insertOffsetRows}[4]{
\multirow{#2}{3cm}{\textbf{#1}}
\csvreader[head to column names,
           late after line=\\\cline{2-5},
           filter expr={
               test{\ifnumgreater{\thecsvinputline}{#3}}
               and test{\ifnumless{\thecsvinputline}{#4}}
         }]%
{\filepath}{}%
{\columns }%
}

%-------------------------------------------------------------------------------------------

\newcommand{\maketable}{
\begin{tabular}{|l|l||l|l|l|}%
\hline
\multicolumn{5}{|c|}{\textbf{\tabletitle}} \\
\hline
\insertRows{General}{2}{4}
\hline
\hline
%------------------------------------------------------
\insertOffsetRows{Environment Properties}{5}{3}{9}
\hline
\hline
%------------------------------------------------------
\insertOffsetRows{Observation Properties}{4}{8}{13}
\hline
\hline
%------------------------------------------------------
\insertOffsetRows{Action Properties}{4}{12}{17}
\hline
\hline
\end{tabular}}

%-------------------------------------------------------------------------------------------


==> inc/makeenvtable6.tex <==
\usepackage{csvsimple,filecontents}
\usepackage{multirow}
\usepackage{xstring}
\usepackage{amsfonts}
\usepackage{amsmath}

\newcommand{\xmark}{\text{\sffamily X}}
\newcommand{\convert}[1]{%
    \IfEqCase{#1}{%
        {Y}{\checkmark}%
        {N}{\xmark}%
        {C}{$\nearrow$}%
        % you can add more cases here as desired
    }[\textbf{#1}]% Assumption, if it is not one of the above cases, then it is a header...
}%
\newcommand{\pconvert}[1]{%
    \IfEqCase{#1}{%
        {Name}{\textbf{Name}}%
        % you can add more cases here as desired
    }[#1] % Return unmodified 
}%

%-------------------------------------------------------------------------------------------

\providecommand{\insertRows}[3]{
\multirow{#2}{3cm}{\textbf{#1}} 
\csvreader[head to column names, 
           late after line=\\\cline{2-6},
           filter expr={
           test{\ifnumless{\thecsvinputline}{#3}}
         }]%
{\filepath}{}%
{\columns}%
}

%-------------------------------------------------------------------------------------------

\providecommand{\insertOffsetRows}[4]{
\multirow{#2}{3cm}{\textbf{#1}}
\csvreader[head to column names,
           late after line=\\\cline{2-6},
           filter expr={
               test{\ifnumgreater{\thecsvinputline}{#3}}
               and test{\ifnumless{\thecsvinputline}{#4}}
         }]%
{\filepath}{}%
{\columns }%
}

%-------------------------------------------------------------------------------------------

\newcommand{\maketable}{
\begin{tabular}{|l|l||l|l|l|l|}%
\hline
\multicolumn{6}{|c|}{\textbf{\tabletitle}} \\
\hline
\insertRows{General}{2}{4}
\hline
\hline
%------------------------------------------------------
\insertOffsetRows{Environment Properties}{5}{3}{9}
\hline
\hline
%------------------------------------------------------
\insertOffsetRows{Observation Properties}{4}{8}{13}
\hline
\hline
%------------------------------------------------------
\insertOffsetRows{Action Properties}{4}{12}{17}
\hline
\hline
\end{tabular}}

%-------------------------------------------------------------------------------------------


==> inc/makeenvtable7.tex <==
\usepackage{csvsimple,filecontents}
\usepackage{multirow}
\usepackage{xstring}
\usepackage{amsfonts}
\usepackage{amsmath}

\newcommand{\xmark}{\text{\sffamily X}}
\newcommand{\convert}[1]{%
    \IfEqCase{#1}{%
        {Y}{\checkmark}%
        {N}{\xmark}%
        {C}{$\nearrow$}%
        % you can add more cases here as desired
    }[\textbf{#1}]% Assumption, if it is not one of the above cases, then it is a header...
}%
\newcommand{\pconvert}[1]{%
    \IfEqCase{#1}{%
        {Name}{\textbf{Name}}%
        % you can add more cases here as desired
    }[#1] % Return unmodified 
}%

%-------------------------------------------------------------------------------------------

\providecommand{\insertRows}[3]{
\multirow{#2}{3cm}{\textbf{#1}} 
\csvreader[head to column names, 
           late after line=\\\cline{2-7},
           filter expr={
           test{\ifnumless{\thecsvinputline}{#3}}
         }]%
{\filepath}{}%
{\columns}%
}

%-------------------------------------------------------------------------------------------

\providecommand{\insertOffsetRows}[4]{
\multirow{#2}{3cm}{\textbf{#1}}
\csvreader[head to column names,
           late after line=\\\cline{2-7},
           filter expr={
               test{\ifnumgreater{\thecsvinputline}{#3}}
               and test{\ifnumless{\thecsvinputline}{#4}}
         }]%
{\filepath}{}%
{\columns }%
}

%-------------------------------------------------------------------------------------------

\newcommand{\maketable}{
\begin{tabular}{|l|l||l|l|l|l|l|}%
\hline
\multicolumn{7}{|c|}{\textbf{\tabletitle}} \\
\hline
\insertRows{General}{2}{4}
\hline
\hline
%------------------------------------------------------
\insertOffsetRows{Environment Properties}{5}{3}{9}
\hline
\hline
%------------------------------------------------------
\insertOffsetRows{Observation Properties}{4}{8}{13}
\hline
\hline
%------------------------------------------------------
\insertOffsetRows{Action Properties}{4}{12}{17}
\hline
\hline
\end{tabular}}

%-------------------------------------------------------------------------------------------


==> inc/reportincs.tex <==
%--------------------------------------
% Report specific packages
\usepackage[numbers]{natbib} 
\usepackage{graphicx,subfig}
\usepackage[T1]{fontenc}
\usepackage{changepage}
\usepackage{tcolorbox}
\usepackage{todonotes}
\usepackage{hyperref}
\usepackage{datatool}
\usepackage{graphicx}
\usepackage{multirow}
\usepackage{thmtools}
\usepackage{minted}
\sloppy % to prevent margin overflow
% ----------------------------------
% New commands
\input{inc/newcommands}
\newcommand{\WP}{Wolpertinger\xspace}
\newcommand{\report}{report\xspace} 
\newcommand{\Z}{\mathcal{Z}}
\newcommand{\R}{\mathcal{R}}
\newcommand{\state}{s}
\theoremstyle{definition}
\setcitestyle{citesep={;}}


==> sections/action_approaches/slates.tex <==
%
Here we observed that approaches belonging to the above 
categories were often evaluated on recommender systems,
\ie Slate-MDPs (\autoref{sec:slateMDPs}).
%
%Despite offering an interesting problem formulation Slate-MDPs 
%have not received a considerable amount of attention from the 
%RL community~\citep{afsar2022reinforcement}.
%
%However, the works that we have found on Slate-MDPs use the 
%same principles of the categories outline here. 
%
%Therefore, each section will also feature an evaluation of
%approaches from each respective category for recommendation
%systems. 
%
As outlined in \autoref{sec:slateMDPs}, a Slate-MDP confronts 
learners with an action space $\actions$ that represents the set of all 
possible recommendation slates $\bm{\action}$.
%
Assuming a fixed catalog of recommendable items $\I$, there are
$\binom{|\I|}{k} \times k!$ ordered $k$-sets from which an agent can chose 
from~\citep{ie2019reinforcement}~\footnote{A fixed catalog is a strong assumption. 
Many application domains are dynamic with respect to $|\I|$, 
\eg hosts joining and leaving a network.}.
%
Therefore, Slate-MDPs confront \RL agents with the following 
three challenges~\citep{ie2019reinforcement}:
% 
\begin{itemize}
\item \textbf{Exploration:} For sufficient large set of items $\I$,
executing every possible slate even once for a given state $x$ is 
infeasible.
%
\item \textbf{Generalizability:} For value estimates to generalize 
across slates for an item $i \in \I$, principled compressed representation 
most be found. 
%
\item \textbf{Latency:} Relevant application areas are typically systems expected 
to deliver recommendations within milliseconds. Solutions are required 
that can solve the combinatorial problem of finding an optimal slate with minimal
delay.
\end{itemize}
%
In this section we shall discuss approaches designed for Slate-MDPs and consider
them with respect to the above criteria.
%
Broadly, the approaches that we have found can be assigned to one of the following
categories with respect to addressing the high-dimensional action problem: 
%
\begin{itemize}
\item \textbf{Slate Decomposition} -- the decomposition of (on-policy) Q-functions~\citep{ie2019reinforcement};  
\item \textbf{Proto action} approaches that find nearest neighbours within an embedding space for items $\I$~\citep{sunehag2015deep,10.1145/3240323.3240374,DBLP:journals/corr/abs-1801-00209};  
\item \textbf{Action elimination} that determine which actions can be ignored~\citep{10.1145/3289600.3290999};
\item \textbf{Decomposition approaches} that combine multiple networks for computing a slate~\citep{pmlr-v97-chen19f}.
\end{itemize}


==> sections/action_approaches/summary/curriculum.tex <==
Curriculum learning is a class of reinforcement learning approach
that confronts agent with a sequence of intermediate tasks
-- \ie a curriculum -- that typically increase in complexity as
the agent progresses~\cite{bassich2020curriculum,bassich2019continuous}.
%
Carefully designed curricula have been shown to improve the learning speed and
performance of agents, and have also been applied to the problem of learning 
in large action spaces, \eg through initially learning a small sub-set of 
selected actions, and gradually expanding the number of actions available to the
agent~\cite{pmlr-v119-farquhar20a}.

%"When a desired behaviour is sufficiently complex, or the environment too unforgiving, it can be intractable to learn from
%scratch through random exploration. Instead, by “starting
%small” (Elman, 1993), an agent can build skills, representations, and a dataset of meaningful experiences that allow
%it to accelerate its learning. Such curricula can drastically
%improve sample efficiency (Bengio et al., 2009)."~\cite{pmlr-v119-farquhar20a}

%"Typically, curriculum learning uses a progression of tasks or
%environments. Simple tasks that provide meaningful feedback to random agents are used first, and some schedule
%is used to introduce more challenging tasks later during
%training (Graves et al., 2017). However, in many contexts
%neither the agent nor experimenter has such unimpeded con
%trol over the environment. In this work, we instead make
%use of curricula that are internal to the agent, simplifying
%the exploration problem without changing the environment.
%In particular, we grow the size of the action space of reinforcement learning agents over the course of training"
%~\cite{pmlr-v119-farquhar20a}



==> sections/action_approaches/summary/decomp.tex <==
This class of approaches typically models 
the single-agent problem as a Dec-POMDP
with a composite action space~\cite{9507301}.
%
There are a range of interesting approaches that utilize this formation, including branching
dueling networks, where each branch of the network fulfills the function of an actuator~\cite{tavakoli2018action}, 
and cascading neural networks where the outputs from individual networks are algebraically combined into the 
identifier of the desired action~\cite{tran2022cascaded}. 
%
However, these action decomposition approaches all rely on the principles of multi-agent reinforcement 
learning, and as such required considerations with respect to overcoming multi-agent learning pathologies,
typically reducing the likelihood of (near-)optimal joint policies being obtained.
%
Our detailed summary of each approach from this category will therefore consider the scalability of the 
approach from the perspective of multi-agent learning and the extent to which the selected multi-agent
reinforcement learning approach can overcome the learning pathologies found in these settings.  


==> sections/action_approaches/summary/elimination.tex <==
Action elimination approaches are implemented with 
a module that determines which actions are redundant or irrelevant for given
observation. 
%
This can range from simple approaches, such as excluding the actions with the smallest
logits values emitted from an actor~\cite{10.1145/3289600.3290999} to having an action elimination network
that has been trained to eliminate irrelevant actions using a linear contextual bandit 
module~\cite{zahavy2018learn}.


==> sections/action_approaches/summary/hierarchical.tex <==
Hierarchical approaches also decompose action selection problem into a multi-policy approach,
similar to the action decomposition approach discussed above.
%
However, we consider an approach as hierarchical when the action of one policy is fed into,
and thereby determines, the action selected by a sub-policy, or alternatively, selects
the sub-policy that will be utilized.
%
This approach has some overlap with the action decomposition literature, as indeed,
some approaches there make use of this formulation.
%
The formulation is particularly relevant for PA-MDPs, \eg where one policy is 
responsible for selecting the discrete action that needs to be taken, and
a second continuous policy determines the set of parameters~\cite{wei2018hierarchical}.
%
It is worthy noting that there can be an overlap here with the category of 
hierarchical-agent action decomposition approaches.
%
Indeed, work by Tran et al.~\cite{tran2022cascaded} on deep cascaded reinforcement 
learning agents was first released under a different title: \say{Deep hierarchical 
reinforcement agents for automated penetration testing}~\cite{tran2021deep}, 
with emphasis on the approach utilizing a hierarchically-structured action space
remaining. 


==> sections/action_approaches/summary/proto.tex <==
The idea behind proto action based architectures is to leverage prior domain knowledge about the 
actions and to embed them in a continuous space, over which an actor with a continuous
output can generalize, building on the actor-critic framework~\cite{dulac2015deep}. 
%
Specifically, the approach utilized DDPG~\cite{lillicrap2015continuous}
to propose a \emph{proto action} within the continuous action embedding space. 
%
The $k$-nearest neighbours to the action are subsequently selected, and passed along
with the observation to the critic, which subsequently predicts the utility 
for each action, to refine the actor's choices. 
%
An illustration of the Wolpertinger Architecture adapted from~\cite{dulac2015deep}
can be found in \autoref{fig:actions:proto}. 


==> sections/additional_envs.tex <==
\subsection{Extensive summary of environments} \label{appendix:env_summary}

Below we provide a summary of the evaluation domains that we encountered
while conducting our literature review. 
%
The majority of the domains did not meet all three of our criteria
with respect to confronting learners with the same challenges 
as \aco, namely: high-dimensional action and state spaces,
as well as being adversarial.
%
Nevertheless, the domains are useful for evaluating approaches
for these problems individually (or sometimes more). 
%
We also argue that: i.) there is a need in this area of 
the literature for a benchmarking suit with a standard
set of challenges that approaches can be benchmarked on,
and ii.) even single agent domains can be converted
into adversarial domains through the addition of 
an adversarial \say{nature} agent, giving rise
to \emph{robust adversarial reinforcement learning}\cite{pinto2017robust}.
%
This can be in the form of domain modifications, or simply through 
the adversary perturbing the protagonist agent's actions.

\subsubsection{Gridworlds} \label{app:envs:sub:gridwolrds}

\begin{table}[h]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ |p{3cm}||p{6cm}|p{1.5cm}|p{1.5cm}|p{1cm}|p{1cm}|}
 \hline
 \multicolumn{6}{|c|}{\textbf{Environments Overview}} \\
 \hline
 \textbf{Name} & % Name of the aglo
 \textbf{Description} &  % Wolpertinger | Action Decomposition | Action Elimination | Hierarchical 
 \textbf{HD-$\states$}  &  % Brief summary of the approach
 \textbf{HD-$\actions$}  &  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
 \textbf{Adv.} &  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
 \textbf{Code} \\  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
\hline
\hline
\multicolumn{6}{|c|}{\textbf{Gridworld Domains / 2D Games}} \\
\hline
Categorised $N$-Rooms~\cite{zahavy2018learn} & Gridworld domain where states are randomly assigned to $k$ categories. The agent is tasked with reaching a goal position, but can only move if it takes an action with the correct category. There are therefore $4k$ actions. The move is random with a probability 0.75 if the category is correct, otherwise 0.5. & \xmark & \checkmark & \xmark &  \xmark \\
\hline
\textbf{Selective Predator-Prey}~\cite{song2019solving} & Multiple predators are tasked with capture randomly moving preys (although for adversarial learning one could imagine learning prey). The agent observes the position of all agents (predators and prey), selects $K$ predators, and assigns commands. A reward is given when two predators catch a prey. & \boldcheckmark & \boldcheckmark & \boldcheckmark & \boldcheckmark~\tablefootnote{\url{https://github.com/DeUmbraTX/practical_rllib_tutorial/blob/main/your_rllib_environment.py}} \\
\hline
Multi-Step Plan Environment~\cite{dulac2015deep} &  Construct an $n$-step plan using all possible actions across $n$ steps, \ie the agent has $i$ actions available at each time step and an agent needs to plan $n$ time steps into the future. & \xmark & \checkmark & \xmark & \xmark \\
\hline
Platform Jumping~\cite{wei2018hierarchical} & Simple 2d game in which an agent must move and jump across platforms while avoiding enemies. & \xmark & \checkmark & \xmark & \xmark \\
\hline
\hline
\end{tabular}}
\caption{An overview of evaluation environments and their properties with respect to the 
defined suitable environment criteria. In this table the columns HD-$\states$ and HD-$\actions$ 
refer to state and action spaces that are intractable for traditional reinforcement 
learning approaches, while Adv. denotes adversarial environments.}
\label{tab:environments:gridworlds}
\end{table}

Gridworld domains are frequently observed within the reinforcement learning literature
as means to conduct preliminary evaluations to verify that an approach has some merit.
%
They provide a low-threshold means through which to construct scenarios 
that have relevant properties comparable to an intended target domain. 
%
Due to their popularity, there are numerous repositories available online that allow
one to specify gridworld scenarios with ease~\footnote{\url{https://github.com/bjkomer/gym-maze}}. 
%
Gridworlds have also provided a means through which to construct evaluation scenarios 
for approaches designed to address the high-dimensional action space problem. 

\textbf{Selective predator-prey:} 
%
Song et al.~\cite{song2019solving} propose a selective predator-prey
scenario that involves multiple predators that have to capture randomly moving 
preys that are distributed throughout the environment.
%
The environment is fully observable from the perspective of the agent, who must
at east time step select $K$ predators and assign each a command (the direction
to move in). 
% 
Only the selected predators move according to the selected actions, and capture 
the prey.
%
In addition, two predators must pounce on the prey in order for a reward to be obtained.
%
The domain is interesting in that it features a high-dimensional combinatorial action space,
and also, depending on the domain configuration, potential challenges with respect to 
the dimensionality of the observation space.
%
In a  sufficiently sized grid, feeding the agents the complete observation space will 
likely not be feasible, and therefore other representations would need considering 
(\eg graph based, or partial observations). 
%
Finally, Song et al.~\cite{song2019solving} had randomly moving prey, in principle their
movements could also determined by a learning agent (or multiple-learning agents), adding
an adversarial dimension to this game. 

\textbf{Categorised $N$-Rooms:}
%
In this domain, introduced by Zahavy~\cite{zahavy2018learn}, the 
agent is situated within a gridworld with $N$ rooms. 
%
The agent is tasked with reaching a goal cell, receiving a penalty 
after each step, and a reward of 0 upon reaching the goal.
%
The agent can move in four directions (up, down, left, right).  
%
However, the task is complicated by the fact that each state of the
game is randomly devided into $K$ categories at the start. 
%
At each step the agent must choose among $4 \times K$ actions.
%
The agent will move in the intended direction with a probability
of 0.75 if the correct category is selected.
%
Otherwise the probability is 0.5.


\textbf{Platform Jumping:} 
%
Confronts learners with a Parameterized-Action MDP, 
where an agent must jump across platforms while 
avoiding avoiding enemies~\cite{wei2018hierarchical}.
%
Discrete actions in this domain represent run, jump (over
enemies) and leap (across platforms), 
while the continuous action is speed.  

\textbf{Multi-Step Planning:} 
%
The multi-step planning problem confronts the agent with the challenge of having to 
construct an $n$-step plan using all possible actions across the next $n$ steps~\cite{dulac2015deep}.
%
As result, if the agent can choose among $i$ actions, and needs to plan $n$ steps
into the future, there are $i^n$ possible actions.
%
The authors implement problem setting on a puddle world environment, 
where each cell can have four types: empty, puddle, start, or goal. 
%
A reward of $-1$ is obtained for visiting an empty cell, $-3$ for visiting 
a puddle, and $250$ upon reaching the goal. 

\subsubsection{Domains with graph-based states}

\begin{table}[h]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ |p{3cm}||p{6cm}|p{1.5cm}|p{1.5cm}|p{1cm}|p{1cm}|}
 \hline
 \multicolumn{6}{|c|}{\textbf{Environments Overview}} \\
 \hline
 \textbf{Name} & % Name of the aglo
 \textbf{Description} &  % Wolpertinger | Action Decomposition | Action Elimination | Hierarchical 
 \textbf{HD-$\states$}  &  % Brief summary of the approach
 \textbf{HD-$\actions$}  &  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
 \textbf{Adv.} &  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
 \textbf{Code} \\  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
\hline
\hline
\multicolumn{6}{|c|}{\textbf{Domains with graph-based States}} \\
\hline
DinerDash~\cite{chen2020dinerdash} & A waitress agent is tasked with running a restaurant via a large combinatorial action space. & \xmark & \checkmark & \xmark & \checkmark~\tablefootnote{\url{https://github.com/AdaCompNUS/diner-dash-simulator}} \\
\hline
\end{tabular}}
\end{table}



\textbf{DinerDash}:
Chen et al.~\cite{chen2020dinerdash}
introduce a gym environment where the agent is 
tasked with running a restaurant through controlling a waitress.
%
The objective is to serve as many customers as possible. 
%
The domain configuration illustrated in \cite{chen2020dinerdash} 
has the waitress serving six tables of different sizes and up to 
seven waiting groups. 
%
The size of the groups can vary.
%
The agents actions consist of: 
allocating each group to a table; 
collecting orders; 
submitting orders;
picking up food;
collecting bills;
cleaning the tables;
and returning dishes to the dish collection point.
%
Rewards are determined by a happiness value for each group
of customers.
%
The happiness value will decrease if the customers wait for too long, 
and once the happiness value reaches zero, the customer will leave.
%
This results in the player losing a life -- each episode starts with the
player having five lives.
%
The configuration depicted in \cite{chen2020dinerdash} has a 40 
dimensional state space, and 57 actions.
%
Although given the problem definition, scaling up the scenario
to a larger state and action space is feasible, \eg, through 
increasing the number of tables, adding addition.

\subsubsection{Discretised Continuous Control Domains} \label{Sec:DCCD}

\begin{table}[h]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ |p{3cm}||p{6cm}|p{1.5cm}|p{1.5cm}|p{1cm}|p{1cm}|}
 \hline
 \multicolumn{6}{|c|}{\textbf{Environments Overview}} \\
 \hline
 \textbf{Name} & % Name of the aglo
 \textbf{Description} &  % Wolpertinger | Action Decomposition | Action Elimination | Hierarchical 
 \textbf{HD-$\states$}  &  % Brief summary of the approach
 \textbf{HD-$\actions$}  &  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
 \textbf{Adv.} &  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
 \textbf{Code} \\  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
\hline
\multicolumn{6}{|c|}{\textbf{Discretised Continuous Control Domains}} \\
\hline
\textbf{Discretised Continuous Control Domains}~\cite{tavakoli2018action,gupta2017cooperative,metz2017discrete} & Typically discretised MuJoCo domains. Domains could in principle be made adversarial by incorporating ideas from the robust adversarial reinforcement learning literature~\cite{pinto2017robust,zhang2020stability,dennis2020emergent}~\footnote{Arguably robust adversarial reinforcement learning (RARL) could be applied to most of the domains here. However, RARL is particularly relevant for continuous control domains, where it has a strong track record of improving the robustness of agents.}. Can in principle also include high-dimensional observation spaces.  & \boldcheckmark & \boldcheckmark & \boldcheckmark & \boldcheckmark~\tablefootnote{MuJoCo continuous control domains are available within the Open AI Gym (\url{https://github.com/openai/gym}). Cooperative multi-agent continuous control domains are available via the PettingZoo (\url{https://pettingzoo.farama.org/environments/sisl/})}  \\
\hline
\hline
\end{tabular}}
\end{table}

Discretised continuous control domains (\eg., environments
are simulated using the MuJoCo physics engine~\cite{todorov2012mujoco})
have become a popular means through which to obtain
high-dimensional MultiDiscrete action spaces for 
evaluating proposed approaches~\cite{dulac2015deep,tavakoli2018action}.
%
Within these domains each action dimension $d = \{1, ...,N\}$ of the original continuous
control action space is discretized into $i$ segments, resulting
in an action space with $\rvert\actions\rvert = i^d$ actions~\cite{dulac2015deep,tavakoli2018action}.
%
Depending on the granularity of the discretization, one can 
construct intractable action spaces with ease within these domains,
as demonstrated in \autoref{tab:disc_cont_envs}, listing the
number of combinatorial actions with a discretization of $n=33$
actions for each actuator. 
%
\begin{table}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ |p{2.5cm}||p{7cm}|p{4cm}|p{5cm}|} %p{3cm}|   }
 %\hline
 %\multicolumn{4}{|c|}{Discretized Continuous Environments - Domain Properties} \\
 \hline
 \textbf{Domain} & \textbf{Observation Space Dimension dim($o$)} & \textbf{Action Dimensions $N$} & \textbf{$n^N$ combinatoral actions} \\ %& BDQ Network Outputs ($n \times N$) \\
 \hline
 Reacher-v1    & 11  & 2 & $1.1 \times 10^3$ \\% & 66\\
 Hopper-v1     & 11  & 3 & $3.6 \times 10^4$ \\% & 99\\
 Walker2d-v1   & 17  & 6 & $1.3 \times 10^9$ \\% & 198\\
 Humanoid-v1   & 376 & 17 & $6.5 \times 10^{25}$ \\% & 561\\
 \hline
\end{tabular}}
\caption{Dimensionality and number of actions using a granularity of $n=33$, a setting 
used by \cite{tavakoli2018action}.}
\label{tab:disc_cont_envs}
\end{table}

\subsubsection{Text Based Games} \label{sec:text_based_games}

\begin{table}[h]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ |p{3cm}||p{6cm}|p{1.5cm}|p{1.5cm}|p{1cm}|p{1cm}|}
 \hline
 \multicolumn{6}{|c|}{\textbf{Environments Overview}} \\
 \hline
 \textbf{Name} & % Name of the aglo
 \textbf{Description} &  % Wolpertinger | Action Decomposition | Action Elimination | Hierarchical 
 \textbf{HD-$\states$}  &  % Brief summary of the approach
 \textbf{HD-$\actions$}  &  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
 \textbf{Adv.} &  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
 \textbf{Code} \\  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
\hline
\multicolumn{6}{|c|}{\textbf{Text Based Games}} \\
\hline
Zork~\cite{zahavy2018learn} & Zork is a \emph{text-based game} where the agent must interact via a text-based interface, having to choose from over a thousand possible actions per state. & \checkmark & \checkmark & \xmark & \checkmark~\tablefootnote{\url{https://github.com/TomZahavy/CB_AE_DQN}} \\
\hline 
\hline
\end{tabular}}
\end{table}

\textbf{zork} is an interactive text based computer game, created by a member of the MIT Dynamic 
Modeling Group in the late 1970s~\cite{zahavy2018learn}.
%
Given that text-based interactions are required in order for a player/agent to progress,
Zork offers an environment with large state and action spaces, with the later also being
implemented by natural language.
%
A natural language parser processes the text provided by the player, which following 
the sophisticated parsing process is turned into an action and execute.  
%
The game confronts the player with range of challenging puzzles and navigation tasks, 
requiring intricate action sequences to solve.
%
To solve this game an agent must be capable of both long-term planning, and dealing 
with random events, \eg attacks~\cite{zahavy2018learn}.  
%
Suitable network architectures are required for this game that can handle NLP tasks~\cite{zahavy2018learn}. 

\subsubsection{Card Games}

\begin{table}[h]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ |p{3cm}||p{6cm}|p{1.5cm}|p{1.5cm}|p{1cm}|p{1cm}|}
 \hline
 \multicolumn{6}{|c|}{\textbf{Environments Overview}} \\
 \hline
 \textbf{Name} & % Name of the aglo
 \textbf{Description} &  % Wolpertinger | Action Decomposition | Action Elimination | Hierarchical 
 \textbf{HD-$\states$}  &  % Brief summary of the approach
 \textbf{HD-$\actions$}  &  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
 \textbf{Adv.} &  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
 \textbf{Code} \\  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
\hline
\hline
\multicolumn{6}{|c|}{\textbf{Card Games}} \\
\hline
DouDizhu~\cite{pmlr-v139-zha21a} & Three-player card game where two players have to team up against a landlord. The game features a large action space with 27,472 possible combinations. &  \xmark & \checkmark & \checkmark & \checkmark~\tablefootnote{\url{https://github.com/kwai/DouZero}~\tablefootnote{\url{https://github.com/kwai/DouZero}}} \\
\hline
\hline
\end{tabular}}
\end{table}

\textbf{DouDizhu} is a three-player shedding-type card game, where the objective is
for each player to empty their hand before the other players~\cite{pmlr-v139-zha21a}.
%
In this game two players (termed Peasants) must team up against a Landlord. 
%
The Peasants win if either of them is the first to have no cards left before the landlord.  
%
This game is challenging due to i.) the two Peasants having to learn to coordinate,
and ii.) the 27,472 card combinations, representing the action space~\cite{pmlr-v139-zha21a}.
%
Different subsets of actions are legal depending on the current hand.
%
There is no easy way to abstract the action space, as playing an improper card can result
in an instant loss~\cite{pmlr-v139-zha21a}.  

\subsubsection{Networks}

\begin{table}[h]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ |p{3cm}||p{6cm}|p{1.5cm}|p{1.5cm}|p{1cm}|p{1cm}|}
 \hline
 \multicolumn{6}{|c|}{\textbf{Environments Overview}} \\
 \hline
 \textbf{Name} & % Name of the aglo
 \textbf{Description} &  % Wolpertinger | Action Decomposition | Action Elimination | Hierarchical 
 \textbf{HD-$\states$}  &  % Brief summary of the approach
 \textbf{HD-$\actions$}  &  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
 \textbf{Adv.} &  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
 \textbf{Code} \\  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
\hline
\multicolumn{6}{|c|}{\textbf{Networks}} \\
\hline
Intelligent Communication Jamming~\cite{e24101441} & Communication jamming decision making domain where two communication parties can adjust physical layer parameters to avoid jamming in a non-cooperative scenario.  & \xmark & \checkmark & \checkmark & \xmark \\
\hline
Multicast Scheduling Problem~\cite{li2022multicast} & The multicast scheduling problem requires the broadcasting of multiple messages over multiple channels. The objective is to minimizes the energy consumption of the base station and the latency of serving asynchronous requests from the mobile users. & \xmark & \checkmark & \xmark & \xmark \\
\hline
\end{tabular}}
\end{table}


\textbf{The Multicast Scheduling Problem:} 
%
Multicasting is a technique for efficiently transmitting common message from a base station 
to multiple mobile users in parallel~\cite{li2022multicast}.
%
The multicast scheduling problem consists of sending multiple message through multiple channels,
while simultaneously reducing the energy consumption of the base station, and reducing the latency
with which mobile users receive the messages.
%
The challenge is made more challenging due to requires being asynchronous.
%
The problem is challenging due to a large action space that must satisfy time-varying constraints.  

\textbf{Intelligent Communication Jamming:} 
%
Xu et al.~\cite{e24101441} study an intelligent jamming decision electronic warfare scenario,
in which two communication agents must adjust physical layer parameters to avoid blocking by
a jammer.
%
The scenario is considered from the perspective of the jammer (although in principle RL
could also be applied to the sender and receiver agents).
%
The domain features a MultiDescrete action spaces as must adust communication 
parameters including, modulation $\{M_1, M_2, ..., M_n\}$, transmission power 
$\{P_1, P_2, ..., P_m\}$ and communication frequency points $\{C_1, C_2, ..., C_l\}$.
%
The scenario is depicted in~\autoref{fig:jaming}.
%
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{img/envs/jamming.png}
\caption{Depiction of an intelligent communication jamming architecture (adopted from~\cite{e24101441}).}
\label{fig:jaming}
\end{figure}

\subsubsection{Recommender Environment} \label{sec:env:recommender_envs}

\begin{table}[h]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ |p{3cm}||p{6cm}|p{1.5cm}|p{1.5cm}|p{1cm}|p{1cm}|}
 \hline
 \multicolumn{6}{|c|}{\textbf{Environments Overview}} \\
 \hline
 \textbf{Name} & % Name of the aglo
 \textbf{Description} &  % Wolpertinger | Action Decomposition | Action Elimination | Hierarchical 
 \textbf{HD-$\states$}  &  % Brief summary of the approach
 \textbf{HD-$\actions$}  &  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
 \textbf{Adv.} &  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
 \textbf{Code} \\  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
\hline
\multicolumn{6}{|c|}{\textbf{Recommender Environments}} \\
\hline
Recommender Environment~\cite{rohde2018recogym,2021RL4RS,pmlr-v97-chen19f,10.1145/3289600.3290999,ie2019reinforcement,afsar2022reinforcement} & Recommender systems where the agent is required to suggest a list (or a page) of options. See the section on Slate-MDPs for a formal definition of this problem~\autoref{sec:slateMDPs}. & \checkmark & \checkmark & \xmark & \checkmark~\tablefootnote{\url{https://github.com/fuxiAIlab/RL4RS}, \url{https://github.com/criteo-research/reco-gym}}\\
\hline
\hline
\end{tabular}}
\end{table}

While the Slate-MDP problem formulation could be relevant for a 
range of application areas -- \eg human-in-the-loop \aco environments -- 
the majority of works in this area are implemented for and
evaluated on recommendation systems
~\cite{pmlr-v97-chen19f,10.1145/3289600.3290999}.
%
The recommender system problem can essentially be formulated as follows:
given a huge corpus of content, can we find an efficient policy small
fractions of content that a user will be interested in~\cite{10.1145/3289600.3290999},
e.g., TV show recommendations on Netflix and Amazon.
%
Taking into account user preferences here is the key, as recommender 
systems are tasked with recommending the right item, to the
right user, at the right time.
%
Again, relating to \aco, given a group of specialised administrators,
 a recommender system could be tasked with flagging up activities 
that it deems suspicious to the admin who is most interested (and
most likely to resolve identify and solve the matter).
%
A key component of the recommender system training process
is that the user provides feedback through an action from 
the slate being selected and executed, \ie the movie is played
for a certain duration.
%
Based on this feedback the system can adjust its model and make
further recommendations.
%
Put simply, at each time step, the system displays $k$ items
(presenting a slate of $k$ actions), the user then picks an action,
feedback is provided, the system moves on to the next state, and
a new slate based is made~\cite{pmlr-v97-chen19f}. 
%
In industrial settings recommender systems are confronted 
with large state and action spaces, due to the large number 
of items from which to select recommendations.
%
To complicate the matter the set of items from which the agent
can choose a slate is often non-stationary,
and often growing, leading to an ever larger action space~\cite{10.1145/3289600.3290999}.
%
User preferences are also non-stationary thereby introducing 
drift~\cite{10.1145/3289600.3290999}.
%
The observation space is large, as it can feature both static
features, \eg demographic, declared interests, and other attributes, as well
as context (time of the day, user location), and encodings of past behaviour.
%
Efficient methods are therefore required for encoding a user's history.
%
The scenario is depicted in \autoref{fig:recomendation_system}.
%
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{img/envs/recomendation_system.png}
\caption{Depiction of a recommendation system (adopted from~\cite{pmlr-v97-chen19f}).}
\label{fig:recomendation_system}
\end{figure}

\subsubsection{Fully Cooperative Multi-Agent Environments}

\begin{table}[h]
\resizebox{\columnwidth}{!}{
\begin{tabular}{ |p{3cm}||p{6cm}|p{1.5cm}|p{1.5cm}|p{1cm}|p{1cm}|}
 \hline
 \multicolumn{6}{|c|}{\textbf{Environments Overview}} \\
 \hline
 \textbf{Name} & % Name of the aglo
 \textbf{Description} &  % Wolpertinger | Action Decomposition | Action Elimination | Hierarchical 
 \textbf{HD-$\states$}  &  % Brief summary of the approach
 \textbf{HD-$\actions$}  &  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
 \textbf{Adv.} &  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
 \textbf{Code} \\  % MDPs, POMDPs, Slate-MDPs, Dec-POMDPs, etc
\hline
\multicolumn{6}{|c|}{\textbf{Fully Cooperative Multi-Agent Environments}} \\
\hline
PettingZoo~\cite{terry2021pettingzoo} & Library featuring numerous domains that could be viewed through the lense of applying a single agent joint-action learning approach to domains with a MultiDescrete action space. & \checkmark & \checkmark & \xmark & \checkmark\tablefootnote{\url{https://pettingzoo.farama.org/}} \\
\hline
SMAC~\cite{samvelyan2019starcraft,samvelyan19smac} & Benchmarking environment based on the popular real-time strategy game StarCarft II. & \boldcheckmark & \boldcheckmark & \boldcheckmark & \boldcheckmark\tablefootnote{\url{https://github.com/oxwhirl/smac}} \\
\hline
Traffic Simulations~\cite{lopez2018microscopic} & Microscopic Traffic simulation tool for traffic research. Allows for the implementation of complex distributed traffic light control scenarios. & \checkmark & \checkmark & \xmark & \checkmark~\tablefootnote{\url{https://www.eclipse.org/sumo/}} \\
\hline
Iroko~\cite{ruffy2018iroko} & Flexible, configurable emulator for benchmarking data-driven congestion control on networks. & \checkmark & \checkmark & \checkmark & \checkmark\tablefootnote{\url{https://github.com/dcgym/iroko}} \\
\hline
Team-Games~\cite{JMLR:v17:15-417,bloembergen2010lenient,wei2018multiagent,bloembergen2010lenient,palmer2018negative,palmer2018lenient,palmer2020independent}
&
Various team games from the multi-agent reinforcement learning literature designed to evaluate the extent to which approaches are susceptible toward multi-agent learning pathologies. Includes both stateless game, and games with high-dimensional states/observations. 
& \checkmark & \checkmark & \xmark & \checkmark \\
\hline
Half Field Offense~\cite{HFO}
&
Half Field Offense is a soccess simulation where players are either designated as attackers or defenders.
& \checkmark & \checkmark & \checkmark & \checkmark~\tablefootnote{\url{https://github.com/LARG/HFO}} \\
\hline
\end{tabular}}
\end{table}

Many of the MultiDescrete problem scenarios discussed in this 
report can infact the viewed as cooperative learning scenarios,
\eg  
the discretised continuous control domains discussed in \autoref{Sec:DCCD}.
%
Within this scenario each actuator can be viewed as an agent.
%
As we shall see in \autoref{sec:action_decomposition} approaches in this
area are prone to some of the challenges encountered in multi-agent learning.
%
Indeed, the multi-agent learning literature considers single 
agents solutions applied the above problem formulation as joint-actions 
learners, where one agent learns a policy for all agents in the system,
while the alternative is concurrent learning, where agent's learn 
a policy independently~\cite{palmer2020independent}. 
%
Indeed, one of the motivating factors for turning to multi-agent learning
is the notion that, while single agent learning approaches perform well
when applied to joint-action learning problems, the approaches often
do not scale well, as increasing the number of agents results in an 
exponential increase in the size of the observation-action space
~\cite{hernandez2017survey,matignon2007hysteretic,rashid2018qmix,
son2019qtran,sunehag2017value,guptacooperative,
castellini2019representational,devlin2011theoretical}. 
%
Indeed, in action space that allows each of $N$ actoins to 
take an action from a set $\actions_{agent}$ we have an 
exponentially large action space of size $\rvert\\actions_{agent}\rvert^N$.
%
Therefore, the multi-agent learning literature provides a 
numerous environments capable of confronting agents with 
high dimensional observation spaces and high dimensional 
action spaces capable of stress testing approaches designed 
to address these issues. 
%
Below we provide an overview of suitable domains and gym frameworks. 

\textbf{PettingZoo Library:} Terry et al.~\cite{terry2021pettingzoo} introduced 
the PettingZoo library along with an accompanying agent environment cycle games
model, providing a diverse set of multi-agent learning environments with a 
Python API to accelerate multi-agent reinforcement learning research.
%
The motivation for implementing it was to provide a multi-agent reinforcement 
learning equivalent of the OpenAI Gym that is frequently used for single agent
reinforcement learning~\cite{brockman2016openai}. 
%
The library provides a range of domains that can be viewed through the lens
of MultiDiscrete action learning, \eg the cooperative multi-agent control 
domains provided by the Stanford Intelligent Systems Laboratory (SISL) would provide
suitable benchmarking domains for approaches aimed at tackling discretized 
control environments, confronting learners with both a high-dimensional
combinatorial action space and, through the multiple observation points,
a high dimensional observation space
~\footnote{\url{https://pettingzoo.farama.org/environments/sisl/}} (See~\autoref{fig:SISL} 
for a depiction of the relevant domains). 
%
\begin{figure}[h]
\centering     %%% not \center
\subfloat[Mult-Agent Walker]{\label{fig:envs:MAWalker}\includegraphics[height=35mm]{img/envs/MAWalker.png}}
\hspace{5mm}
\subfloat[Pursuit]{\label{fig:envs:Pursuit}\includegraphics[height=35mm]{img/envs/Pursuit.png}}
\hspace{5mm}
\subfloat[Waterworld]{\label{fig:envs:Waterworld}\includegraphics[height=35mm]{img/envs/Waterworld.png}}
\caption{Cooperative multi-agent control benchmark environments introduced by Stanford Intelligent Systems Laboratory (SISL) that would make 
interesting benchmarking domain for discretized control approaches.}
%\label{fig:SISL}
\end{figure}

\textbf{StarCraft Multi-Agent Challenge (SMAC):}
%
SMAC is a partially-observable benchmarking environment based 
on the popular real-time strategy game 
StarCarft II~\cite{samvelyan2019starcraft,samvelyan19smac}.
%
It confronts learners with a micromanagement task, where combat units
are typically controlled by an independent agent that much act based 
on local observations.
%
However, the environment also presents an opportunity for benchmarking
joint-action learners, given that it features many of the properties
that we listed as desirable in \autoref{sec:target_env_properties}, 
including high dimensional action and observation spaces, as well
as the facility for adversarial learning. 
%
It is worth noting that this domain has already been used by 
Farquhar et al.~\cite{pmlr-v119-farquhar20a} for evaluating
a curriculum leanring approach for growing action spaces. 
%
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{img/envs/SMAC.png}
\caption{Screenshots from three SMAC scenarios (adopted from~\cite{samvelyan2019starcraft}).}
\label{fig:SMAC}
\end{figure}

\textbf{Microscopic Traffic Simulation:}
%
Microscopic traffic simulations~\cite{lopez2018microscopic} provide a
valuable tool for research on traffic scenarios, as well as benchmarking
domains the features that match the majority of our requirements, perhaps
with the exception of an adversarial component -- although addressable 
through robust adversarial reinforcement learning, \eg an adversary
capable of \say{sabotaging} a traffic light in a grid. 
%
Interesting scenarios that have been explored in the multi-agent 
reinforcement learning literature include distributed 
traffic light control\cite{pmlr-v139-zimmer21a}, and the use
of multi-agent reinforcement learning to simulate agents with
different levels of aggression~\cite{bacchiani2019microscopic}.

\textbf{Distributed Data Center Control:}
%
Explores the question of whether data-driven congestion control
agents using deep reinforcement learning can learn optimal
network policies.
%
The Iroko emulator allows the benchmarking of approaches in this
setting~\cite{ruffy2018iroko}.
%
Iroko is flexible, allowing the modelling of different network
topologies, congestion and deployment scenarios. 
%
It provides an OpenAI gym interface, and therefore has become
a popular tool for multi-agent reinforcement learning benchmarking~\cite{pmlr-v139-zimmer21a}.

\textbf{Team-Games}
%
As we shall see under approaches for high dimensional action spaces in \autoref{sec:hdas_approaches}, 
one category of methods uses what can be viewed as a multi-agent approach towards composing
a combinatorial action.
%
Authors in this area of the literature have noted that their methodologies can fail to 
learn cooperate and converge upon a reasonable policy when implemented with independent
learning approaches, and as a result turn towards advanced multi-agent reinforcment learning
approaches (\eg QMix~\cite{rashid2018qmix}) to facilitate cooperation.
%
However, this raises the question of the extent to which the resulting implementations are
indeed robust to the multi-agent learning pathologies discussed in \autoref{sec:marl_concepts},
in particular at scale, \ie when the action is the result of a decomposition into a large 
number of agents.
%
Here the multi-agent reinforcement learning literature offers a range of games designed 
to tease out how suceptable an approach is towards a particular sub-set of pathologies.
%
A large number of these games are even stateless, therefore offering focused benchmarking
domains to try out novel approaches for testing the action composition processes
~\cite{JMLR:v17:15-417,bloembergen2010lenient,wei2018multiagent,bloembergen2010lenient}. 
%
Meanwhile, in other work, the same problem formulation has been transolated into 
DecPOMDPs with a compareable reward space~\cite{palmer2018negative}.  



==> sections/discussion.tex <==
\section{Discussion} \label{sec:discussion}

\subsection{The need for improved evaluation environments}

"A key assumption taken by this report is that in a conflict with a technically 
sophisticated adversary, NATO military tactical networks will operate in a heavily 
contested battlefield. Enemy software cyber agents—malware—will infiltrate 
NATO networks and attack NATO C4ISR and computerized weapon systems, with 
a significant probability that cannot be ignored."
\citep{kott2018autonomous} --> Need for environments where battlefield decisions
need to be made along side cyber-defence decisions? CC3-4 a step in the right 
direction, however, DRL defence agents still only control cyber-defence decisions.
Specifically, in CC3 the tracking of troops, and manuvering of the UAVs is 
left to a rules-based swarm algorithm.
%
\comGP{Need to make this part more cyber-defence env specific, highlight the weaknesses of current envs, etc.}
%
In \autoref{sec:envs}, it is identified that the challenges
which would be present in an idealised \aco training environment are not currently
implemented in CybORG\reportonly{, PrimAITE,} or YAWNING TITAN.
%
While \envs are available to benchmark
subsets of these challenges, no environment can be used to benchmark all of them.
%
In particular, although \emph{RecSim} and \emph{Micro-RTS} are available to benchmark
high-dimensional observation and action spaces, respectively, no environment is
available to pose these challenges alongside graph-based dynamics.
%
%Assuming that these dynamics hold some importance in the \aco problem space,
Practitioners aiming to develop methodologies which rely on graph constructs specifically
have several avenues for environment development, with two open-source but difficult to
modify \aco environments being available, alongside frameworks such as \emph{Gym-ANM} which
are designed to be built upon.
%
As such, the following research (and development) questions arise:
%
\begin{description}
\item[\textbf{Q2:}] Will methodologies developed on environments such as \emph{RecSim} and \emph{Micro-RTS} translate well to \aco?
\item[\textbf{Q3:}] Where should environment developers seeking to build towards a more idealised graph-based \aco-like environment focus their efforts?
\end{description}

\subsection{Performance in Real-world Scenarios}

Given the components discussed in this paper,  
be to setup a modular framework that combines the solutions recommended in this review, 
and conducting large scale ablation studies and hyperparameter tuning exercises to evaluate
which approaches work best.
%
An aspect that we have not addressed in this work, 
and that is perhaps not explicit defined within current
cyber-defence environments, is that, 
"in case the enemy malware knows that the agent exists and 
is likely to be present on the computer, the enemy malware will seek to find and 
destroy the agent. Therefore, the agent will possess techniques and mechanisms for 
maintaining a certain degree of stealth, camouflage, and concealment. More 
generally, the agent takes measures that reduce the probability that the enemy 
malware will detect the agent. The agent is mindful of the need to exercise self-preservation and self-defense"
\cite{kott2018autonomous,theron152}
--> Low hanging fruit here would be extending CC3 to allow for self-recovering UAVs, 
with blue cyber-defence agents able to "hide" once the node is compromised, and capable
of taking actions for self-recovery at the danger of being detected.

"The agent shall function under specific circumstances, such as limited 
computing resources (memory, CPU, etc.) and special environmental 
conditions (e.g., temperature, air pressure, G-forces, size, and so on.)"
\cite{kott2018autonomous} --> Need for robust policies that are 
transferable across a range of domain parameterizations. 

The authors list picking nearest neighbours in discretized
 control tasks and spatial locations in settings where the 
policy has to control multiple agents as examples of domain
knowledge for constructing this action hierarchy. 
%
The authors do hypothesis that action-embeddings in 
a latent space could provide a means for clustering 
actions, however, this assume that the action behaviour 
can be captured sufficiently via random behaviour
demonstrations.
%
Therefore, this is left for future work.



















\subsection{Open Research Questions to guide future research}

Throughout this \report we have identified a number of open research questions, including:

This raises the question of what insights could be gained from
applying feature selection to the CAGE Challenges when using
offline \RL.

An evaluation of the extent to which state abstraction can be applied to \aco, and what we can
learn from it, is a question for future research.

With respect to efficient exploration of large state-spaces, how 
to determine which parts of the state space that are most relevant~\cite{pmlr-v134-perdomo21a}?

Indeed, \cite{dulac2015deep} mentioned under opportunities for future
work that learning action representations during training would
be an interesting direction, allowing actions that are poorly 
placed in the embedding space to be moved to other parts. 
\comGP{Need to see if there has been any progress on this!}

Wolptinger:
Indeed, evaluating expressive functions that could represent
an alternative to $k$NN -- \eg beta policies \cite{jerome2022market}
-- represent interesting opportunities for future work. 

Therefore, designing problem formulations to quantify the susceptibility of SOTA action
decomposition approaches towards each of these pahtologies represents an interesting direction
for future research.



CRLA is a powerful formulation, where there are still a large number of 
RQ remain open.

A lot of approaches, but no paper exists currently that compares all of them! The most logical
follow on work from this one would be a benchmarking report, comparing existing approaches
across the \aco domains and those that we have highlighted as interesting.


The fact that independent learners can match the performance of CRLA-QMIX
raises the question if a performance improvement could be achieved by
less parameter heavy optimistic approaches, designed to facilitate 
cooperation among independent learners~\cite{omidshafiei2017deep,palmer2018lenient,palmer2018negative,palmer2020independent},

Evaluating the scalability of CRLA.

CL:



==> sections/executive_summary.tex <==
\section*{Executive Summary}

In this literature review we consider the challenge of applying deep reinforcement 
learning (DRL) to autonomous cyber operations (ACO). 
%
The cyber defence problem features an adversarial game between \blue 
and \red, two agents tasked with defending and attacking network resources
respectively. 
%
There are numerous variations of this problem. 
%
\red objectives can include compromising key operational 
systems (\emph{capture the flag})~\citep{cage_challenge_announcement,cage_challenge_2_announcement} 
or making resources unavailable via \emph{denial of service} (DoS) attacks. 
%
Typically \blue will face the challenge of having to distinguish \red activities
from those performed by non-threatening Green agents, where \blue's actions
must have a minimal impact on Green. 
%
%Networks can also be ad-hoc, \eg formed by a team of autonomous drone hosts~\cite{cage_challenge_3_announcement}. 

\aco lies at the intersection of three open challenges for DRL, namely learning in an 
environment that confronts \blue 
with a high-dimensional state space, 
a large multi-discrete action space, and adversarial learning. %against a 
%(potentially non-stationary) opponent.
%
Each challenge represents an active area of research. 
%
This report provides a survey of the DRL literature, in order
to conceptualize an idealised ACO-DRL agent.
%
It includes:
%
\begin{itemize}
    \item A summary of the domain properties that define the ACO problem;
    \item A comprehensive evaluation of the extent to which environments used for benchmarking DRL approaches are comparable to ACO;
    \item An overview of state-of-the-art approaches for scaling DRL to environments suffering from the curse of dimensionality;
    \item A survey and critique of current methods for limiting the exploitability of agents within adversarial settings from the perspective of ACO.
\end{itemize}
%
%i.) A summary of the domain properties that define the ACO problem;
%%
%ii.) A comprehensive evaluation of the extent to which domains used for benchmarking DRL approaches are comparable to ACO;
%%
%iii.) An overview of state-of-the-art approaches for scaling DRL to domains that confront learners with the curse of dimensionality;
%%
%and, iv.) A survey and critique of current methods for limiting the exploitability of agents within adversarial settings from the perspective of ACO.
%
We conclude with open research questions that we hope will motivate future directions for researchers and practitioners working on ACO.
%
Below we provide a short summary of each contribution.

\textbf{Environments:}
%
The aim of this \report is to critically evaluate the suitability 
of the current state-of-the-art DRL methodologies 
for ACO.
%
The \emph{full} cyber security problem is a challenging domain for autonomous agents, due
to the properties mentioned above.
%
Of particular concern is the fact that 
limiting the exploitability (the extent to which an opponent
can find a new approximate best response) of DRL agents 
is notoriously challenging, in particular
for agents attempting to overcome the \cod
~\citep{lanctot2017unified,gleave2019adversarial,heinrich2016deep,mcaleer2020pipeline}.
%
The majority of papers on \aco problems to-date focus on the high-dimensional action space
challenge; they benchmark approaches against the set of rules-based agents provided by the domain
implementations.
%
However, as mentioned above, in practice the \aco problem is an adversarial game, where the
stationarity of one's opponent is a strong assumption. 
%
%Therefore, approaches are required that not only address the curse-of-dimensionality, but 
%that limit the exploitability, \ie where a new learning adversary
%will struggle to find a best response that improves on current attacks. 
%
%Limiting exploitability is computationally expensive 
%even for relatively simple games, 
%such as poker~\citep{perolat2022mastering}. 
%
%In addition, it has been observed that finding adversarial attacks on DRL agents is 
%easier for high dimensional observation spaces~\citep{gleave2019adversarial}. 
%
Therefore, the \aco domain offers an interesting open challenge for the adversarial learning community. 
%
Given the need for an extensive evaluation of approaches for \aco, in this report we consider 
both existing cyber defence environments for evaluating DRL agents, as
well as the extent to which environments outside of the field of cyber security feature %confront agents with 
the same set of problems.
%
For each domain we provide a description with respect to the task objective, 
and subsequent evaluation of whether it meets an evaluation criteria that we
formulate with respect to \aco domains. 
%
We broadly assign environments to one of the following categories: 
%
gridworld domains and 2D games;
%
discretised continuous control domains; 
%
network-based domains;
%
recommender systems;
%
and miscellaneous games for unique environments, which do not justify an additional category.

\textbf{Coping with very high-dimensional inputs:}
%
While using powerful deep neural networks (DNNs) as function approximators has allowed
the scaling of RL to high-dimensional observation spaces, there are 
still a number of environments that show the current limits of standard DRL approaches. 
%
In this \report we provide a summary of approaches towards tackling the 
curse-of-dimensionality with respect to state spaces, namely:
%
\begin{itemize}
    \item state representation, \eg using a graph-based representation and leveraging graph neural networks (GNNs);
    \item state abstraction, \eg grouping semantically similar states together using an encoder;
    \item exploration, principled approaches towards guaranteeing a sufficient visitation of semantically similar
    state-action pairs; and,
    \item knowledge retention, preventing the catastrophic forgetting of previously learned behaviours/encodings.
\end{itemize}

\textbf{Approaches for combinatorial action spaces:}
%
Due to an explosion in the number of state-action pairs, traditional
DRL approaches do not scale well to environments that require learners
capable of handling a high-dimensional combinatorial action space. 
%
Requirements here include: 
%
\generalizability, the ability to generalize 
over an action space~\citep{dulac2015deep}; 
\unseenactions, for the domains of interest
the action space can grow, \eg a new host added to the
network; and,
Computational Complexity, an idealised approach
should allow for a tractable computation. 
%
In this report we identify a number of approaches that attempt to 
solve the high-dimensional action problem and evaluate them along
the above evaluation axes. 
%
This includes high-dimensional action approaches belonging to the
following five categories: 
%
\begin{enumerate}
    \item \emph{proto action} based approaches;
    \item \emph{action decomposition};
    \item \emph{action elimination};
    \item \emph{hierarchical} approaches; and,
    \item \emph{curriculum learning}.
\end{enumerate}

\textbf{Adversarial Learning:}
%
Before applying approaches from the high-dimensional
state and action space literature to \aco, one needs to consider the above
approaches through the lens of adversarial learning.
%
In this \report we provide a formal definition of the adversarial learning problem, 
along with desirable solution concepts. 
%
We also list solution types, in particular counterfactual
regret and best response approaches.
%
Given that the latter has been applied to adversarial games at scale,
we focus on a particular type of best response approach: 
the approximate double oracle (ADO) approach,
which provides theoretical convergence guarantees within finite zero-sum games.
%
ADO approaches involve iteratively computing an approximate best response
for each player (\blue and \red in our case) against a \emph{mixture} of
existing opponent policies. 
%
We consider the strengths and weaknesses of this approach with \aco's 
curse of dimensionality in mind, and discuss existing solutions towards
scaling \ado approaches. 

\medskip

\noindent We finish with the following recommended directions for future work. 
\begin{itemize}

\item \textbf{Towards improved evaluation metrics for autonomous cyber defence agents.}
%
Current evaluations of agents within cyber defence environments, be they \blue or \red, 
consist of benchmarking approaches against a set of rules-based 
opponents~\citep{cage_challenge_announcement,cage_challenge_2_announcement,cage_challenge_3_announcement,nguyen2020multiple,tran2022cascaded}.
%
However, success achieved against a stationary opponent should be enjoyed with caution.
%
Instead, in this report we advocate for \emph{exploitability} as a more principled metric 
for evaluating the performance of agents for cyber defence scenarios.
%
Here, exploitability refers to the (approximate) best response that a new opponent 
can learn against the fixed policy of the agent being evaluated.
%
Exploitability is a common metric used throughout the adversarial learning literature,
and can be used to measure the extent to which two learning adversaries have 
converged, be it for DRL~\citep{lanctot2017unified} or even for Generative Adversarial 
Networks (GANs)~\citep{oliehoek2018beyond}. 
%
Given that a large number of DRL approaches have been proposed for \aco, the above
consideration regarding evaluation raises the research question:
How exploitable are current approaches for \aco?

\item \textbf{Limiting the exploitability of \aco agents.}
%
Even simple games require
non-trivial approaches in order to reduce exploitability~\citep{lanctot2017unified}.
%
Given that this problem is typically amplified for domains suffering the
curse of dimensionality~\citep{gleave2019adversarial}, 
limiting exploitability within \aco will require a principled approach.
%
Fortunately there exists an entire branch of the RL literature
that focuses on limiting exploitability
~\citep{lanctot2017unified,oliehoek2018beyond,heinrich2016deep,perolat2022mastering,brown2019deep,li2023combining,berner2019dota,vinyals2019grandmaster,liuneupl}. 
%
What all these approaches have in common is that 
%limiting exploitability typically requires
that they typically rely on
the iterative computation of new best responses against an increasingly 
stronger opponent, or ideally a worst-case opponent.
%
This worst-case opponent is rarely present from the start (\eg rules-based opponents
provided within cyber defense benchmarking environments are unlikely to be optimal), 
and will also need to be obtained via an adversarial training procedure. 
%
Therefore, for future work we recommend that that the applicability of current 
solutions from the adversarial literature are considered for \aco.

\item \textbf{Towards the efficient computation of approximate best responses.}
%
As mentioned above, limiting the exploitability of \aco agents will likely
require the iterative computation of a new best response against an opponent
that is also becoming stronger with each iteration.
%
Even in simple games, such iterative best response based approaches can
require a large number of iterations in order to 
converge~\citep{lanctot2017unified,oliehoek2018beyond,heinrich2016deep,perolat2022mastering,brown2019deep,li2023combining,berner2019dota,vinyals2019grandmaster,liuneupl}.
%
For \aco this matter is further complicated by the environment confronting
learners with the curse of dimensionality with respect to both the state
and action space.
%
As we shall discuss in this report at length, learning in such environments
requires non-standard DRL approaches. 
%
Principled methods are required to ensure the 
sufficient visitation of semantically similar state (or observation) 
action pairs.
%
Therefore, in practice, even computing an approximate best response against rules-based 
agents provided by the environment can take anywhere from hours to days.
%
This naturally has implications for approaches where this process has to 
be repeated iteratively against an ever-stronger opponent.
%
This naturally raises the research question: can we find/implement 
\emph{wall time efficient} DRL approaches for \aco?
%
%A sub-question emerges here regarding the extent to 
%which we can improve current SOTA methods for mitigating the 
%\cod.

\item \textbf{What type of game are our Red and Blue agents playing?}
%
Domains where Green agents are present add an interesting twist.
%
The field of game theory typically differentiates between three types of games:
team-games (where the agents all receive the same reward), zero-sum games
(where the reward for \blue would be the negation of the reward for \red) and
general-sum games, that do not meet either of these criteria. 
%
Depending on the reward function, the presence of Green agents can result
in a cyber defence scenario being classed as a general-sum game. 
%
This has implications for the convergence of agents that are attempting
to reduce their exploitability, giving rise to an equilibrium selection 
problem~\citep{omidshafiei2019alpha}.
%
Therefore, the type of game that \blue and \red are playing needs to be
considered to inform the selection of the adversarial learning approach.
%
An exploration of the empirical payoff matrix games that one can discover
when pairing up different \red and \blue agents could give valuable insights
regarding which learning approach to utilize. 
\end{itemize}


==> sections/old_requirements_list.tex <==
\noindent \textbf{Code:} 
%
The availability of %a 
code 
%repository 
%Code base availability is highlighted as desirable, 
%simply because it 
can significantly speed-up research efforts.  %required to make use of the environment.
%
%It is noted that, should significant development efforts be undertaken, then these efforts may be
%best directed towards expanding the open-source \aco environments directly.
%
%As such, 
We only list codeless environments that offer unique properties, 
or require minimal effort to implement. %, %in a low-effort and
%minimalistic manner, 
%are listed in this work.

\spacer
\noindent \textbf{Adversarial:} 
%
%\aco is a (quasi) zero-sum adversarial game where $r_{blue} \approx -r_{red}$.
\comGP{Need to clarify that this box being checked refers to actual adversarial learning.}
\aco is typically an adversarial game between a Blue and a Red agent.
%
%We are therefore keen to identify domains that confront learners with an adversarial learning challenge.

\spacer
\noindent \textbf{General Sum \& Team Games:} 
%
Networks can span multiple geographic locations.
%
%where a single \blue agent is insufficient
%
%not only due to the \cod, 
%but also 
Physical restraints, such as data transmission capacity and latency,  
%
can therefore necessitate a multi-agent reinforcement learning (MARL) approach.
%
%In addition to adversarial learning, the MARL literature also features team-games, 
%where all agents receive a common reward, and general-sum games (all remaining cases).
%
%we desire environments that allow for adversarial training,
%our review also includes multi-agent environments that can be classed as 
%general-sum games and co-operative team-games.
%
%While it is the case that environments with adversarial training specifically are
%desired, several of the environments reviewed are otherwise multi-agent (\eg co-operative) which is
%identified as it will likely be useful to readers, since multi-agent environments universally require
%different approaches to single-agent ones.
%
%Learning to cooperation is non-trivial~\citep{palmer2020independent},
%
%It is possible that multi-agent, non-adversarial challenges 
%may be present in 
%\aco sub-challenges can belong to these categories. 
%
%For instance, networks could span multiple geographic locations.
%
%A single \blue agent will not be able to physically attend to 
%such a network,
%
%not only due to the \cod, 
%but also due to physical
%restraints such as 
%data transmission capacity and latency. 
%
%Here cooperative MARL can provide a solution,
%allowing multi-task learning~\citep{omidshafiei2017deep}, 
%multi-objective learning~\citep{van2014novel},
%ARCD at different levels of granularity,
%and learning communication protocols~\citep{hernandez2018multiagent}.
%\eg networks 
%
%
%For example: %it is possible that 
%multiple agents %may be present on a network 
%performing different tasks on  a network,
%such as performing 
%ARCD at different levels of granularity, or %with different methods or 
%multiple objectives.
%
%It is also possible that 
%As \aco evolves it may %will be 
%In these cases, multiple agents will be required to attend to different sections of the network,
%and it can be anticipated that a level of co-operation and communication between these agents would
%be desired.

\spacer
\noindent \textbf{Stochastic:} 
%
\aco features stochastic factors, \eg 
user activity, equipment failures and the likelihood of a Red attack
succeeding. %, which will present agents with stochasticity.
%The real-world \aco problem features stochastic factors including
%user activity, equipment failures and the likelihood of a Red attack
%succeeding. %, which will present agents with stochasticity.
%
%A level of stochasticity is present in all \aco environments, and is used to represent
%unknown factors which may affect Red and Green activity, such as whether a Red attack succeeds, or the
%variations in Green network traffic.
%
%Therefore, stochasticity is considered a highly desirable property in \aco-applicable \envs.
%
To meet this criteria stochastic state transitions are required.
%
Random starting positions alone are insufficient.
%Note that in this paper we refer to stochasticity in the state transitions of the \env,
%and stochasticity in starting positions only is insufficient to meet this criteria.


\spacer
\noindent \textbf{Graph-Based:} %By the nature of 
With \aco taking place on networks, \acogyms contain underlying
dynamics unique to graph-based domains.
%
%Most notably, 
%In all \acogyms, a Red agent can only move through the network by jumping
%from a node which it has previously compromised to a connected node. 
%
%As such, the topology and connectivity
%of the graph directly influences the behaviour of the Red agent, and therefore the game itself.
%
%Given this, it is desirable that \envs have graph-based dynamics to better represent the challenges
%faced in \aco.
%
%Note that 
Graph-based observation spaces are not necessarily required to fulfil this criteria. % (and indeed, most do not).
%
However, an environment being checked implies the presence of a graph structure. %somewhere within the \env.

\spacer
\noindent \textbf{Multi-Discrete:} Given the high-dimensionality challenge present in both the observation and
action spaces of \acogyms\ -- which increase in size with the number of nodes -- the presence of multiple 
discrete dimensions in the observation and action spaces is highly desirable. %is perhaps the most desirable of all properties.
%
%However, the majority of \envs in other domains have been crafted to avoid or mitigate this
%problem where it naturally appears, and as such, \envs which present an agent with multi-discrete
%observation and action spaces directly are sparse.
%
%Furthermore, by the nature of most domains, multi-discrete observation and action spaces are rarely present
%together, as we shall see in \autoref{sec:envs}. %\comGP{To cut down on text, perhaps end here with ".. as we shall see in \autoref{sec:envs}."?} \comCP{Yes, makes sense}
%
%\chdeleted[id=GP]{For example, since their action spaces are composed of movement in four cardinal directions, (and a few
%extraneous actions which cannot be taken simultaneously with movement) Gridworld \envs rarely have an action
%space more complex than a single discrete choice; conversely, recommender systems contain such a
%large number of actions (as the action space consists of every product available for recommendation) that most
%\envs in this domain have implemented features to vastly reduce and simplify the action space, usually by
%re-framing the problem as a Slate-MDP.}
%
%Factors such as these make environments with multi-discrete observation and action spaces scarce, and therefore
%noteworthy. \comGP{Commented out due to repetition wrt sparse}

\spacer
\noindent \textbf{Extensible Dimension:} %While graph structures being present in the observation and action spaces are
%not listed as essential here, 
%one property of both spaces which results from graph-based dynamics is an
%extensible dimension. 
%
A property of graph-based dynamics is a dimension
that can be expanded to geometrically increase the size of
the composite space, \eg the number of nodes in a network.
%
%This property is included as an inevitable future challenge in \aco: running agents on increasingly large
%networks. 
%
%As such, it is desirable for an \env to be expandable in this way to 
\Envs that meet this criteria allow methodologies
to be tested for scalability to larger observation and action spaces.

\spacer
\noindent \textbf{Continuous Dimension:} As \acogyms scale up, %it is possible that 
a subset of action dimensions might need to be treated as continuous, 
%confronting learners with a PA-MDP,
%will grow so large that treating them as continuous may be necessary.
%
%For example, 
\eg networks featuring a large number of IP addresses. %may be made continuous, 
%should a large number of them prove to be intractable for some \RL approaches.
%
\update{In PrimAITE this is already feasible, 
as the six-dimensional action space for managing firewall settings via an ACL, 
which may pose a challenge to most \RL methods,
contains two dimensions for node IP addresses~\citep{PrimAITE}.}
%
Additionally, continuous attributes may be present in the observation spaces, %for a wide number of reasons, 
representing node vulnerability for example~\citep{YAWNING}.
%
%Already in YT, continuous variables are present in the observation space to represent
%the vulnerability of each node.
%
Therefore, environments with \emph{mixed} input and output types are desirable.
%
%However, the majority of the observation and action spaces in \acogyms are likely to remain
%discrete. 
%
%Therefore, \envs with \emph{entirely} continuous observation or action spaces are undesirable.
%Therefore, the presence of one or more continuous dimensions in the observation and action spaces is identified,
%in order to steer those wishing to develop approaches to handle such mixed input and output types, requiring 
%approaches designed for PA-MDPS.

\spacer
\noindent \textbf{Traditionally Intractable:} %The final desirable property is perhaps the biggest challenge of all.
%
By identifying environments where the observation or action space is intractable, we indicate one of two properties 
that pose a significant, if not impossible, challenge to traditional \RL methodologies:
%
\begin{enumerate}
    \item The multi-discrete space causes an exponential scaling of the size of the space when flattened,
    such that it quickly becomes computationally intractable.
    \item The observation or action space changes in size as a function of the environment;
    %since 
    standard DRL methods % (and deep learning layers in general) \comGP{Commented out, since there is global max pooling that allows for different input sizes. Although apparently does not work well for RL}
    %usually 
    require %that they remain %that their inputs and outputs
    %be of 
    a consistent shape and size. %, such a dynamic can be considered intractable for most \RL approaches.
\end{enumerate}


==> sections/problem_def.tex <==



==> sections/state_approaches/gnns.tex <==
%\subsection{Leveraging Graph Neural Networks} \label{sec:GNNs}


==> sections/state_approaches/implications.tex <==
In this section we have provided an overview of SOTA methods 
to help DRL agents deal with environments that feature
high-dimensional state and observation spaces that even
push SOTA DNNs based approaches to their limits.
%
We have seen while there are a lot of promising approaches, 
questions remain regarding the extent to which the approaches
can be successfully applied to \aco, providing numerous open problems and
 opportunities for future research.
%
We shall now proceed to take a closer look at the current status of
DRL approaches for high-dimensional action spaces, and their applicability
to \aco.


==> sections/target_env.tex <==


